Spectral function of fermions in a highly occupied non-Abelian plasma

We develop a method to obtain fermion spectral functions non-perturbatively in a non-Abelian gauge theory with high occupation numbers of gauge fields. After recovering the free field case, we extract the spectral function of fermions in a highly occupied non-Abelian plasma close to its non-thermal fixed point, i.e., in a self-similar regime of the non-equilibrium dynamics. We find good agreement with hard loop perturbation theory for medium-induced masses, dispersion relations and quasiparticle residues. We also extract the full momentum dependence of the damping rate of the collective excitations.

==> Decomposition.tex <==
\section{Decomposition of the spectral function}
\label{sec:Lor_decompos_rho}

The spectral function can be split into $16$ components, which can be chosen as 
%(see for instance, Juergen Berges' Lecture notes)
\begin{align}
 \label{eq_lorentz_decomp}
 \rho = \rho_S +i\gamma_5 \rho_P + \gamma_\mu \rho_V^\mu + \gamma_\mu \gamma_5 \rho_A^\mu + \frac{1}{2}\,\sigma_{\mu\nu} \rho_T^{\mu\nu},
\end{align}
with the tensor defined as $\sigma_{\mu\nu} = (i/2)[\gamma_\mu, \gamma_\nu]$ and $\gamma_5 = i \gamma^0 \gamma^1 \gamma^2 \gamma^3$. Note that here we used Lorentz indices $\mu,\nu$, which should not be confused with the spin and color indices $\lambda$ and the Dirac indices $\alpha, \beta$, which we used in previous subsections. The components \eqref{eq_lorentz_decomp} can be deduced from the spectral function by projecting
\begin{align}
 \rho_S = \frac{1}{4}\, \Tr\left( \rho \right)\,,& \quad \rho_P = -i\,\frac{1}{4}\, \Tr\left( \rho \gamma_5 \right), \nonumber \\
 \rho_V^\mu = \frac{1}{4}\, \Tr\left( \rho \gamma^\mu \right)\,,& \quad \rho_A^\mu = \frac{1}{4}\, \Tr\left( \rho \gamma_5 \gamma^\mu \right), \nonumber \\
 \rho_T^{\mu\nu} =\,& \frac{1}{4}\, \Tr\left( \rho \sigma^{\mu\nu} \right),
\end{align}
where the trace goes over Dirac indices. Due to the property $\rho^\dagger(y,x) = \gamma^0 \rho(x,y) \gamma^0$, each of the components satisfies $\rho_{\Omega}^{ }(x,y) = \rho_{\Omega}^*(y,x)$ for $\Omega = S,P,V,A,T$. Consequently, the Fourier transform $\rho_{\Omega}(\tcent,\omega,\mbf p)$ of the spectral function with respect to the relative time $\Delta t = x^0-y^0$ is real-valued. 
%Symmetries further simplify the structure. Invariance under a parity transformation forces the pseudo-scalar and axial vector components to vanish $\rho_P = \rho_A^\mu = 0$. 
Due to the underlying symmetries like rotational invariance and parity symmetry, one finds that except for the scalar and vector components the remaining projections vanish, leaving only
\begin{align} 
 \label{eq:rho_decom_reduced}
 \rho(t',t'',p) &= \rho_S + \gamma_\mu \rho_V^\mu \nonumber \\
 &= i\text{Im}\rho_S + \gamma^0 \text{Re}\rho^V_0 + i\gamma^j \text{Im}\rho^V_j\,.
\end{align}
We have checked this numerically in our simulations. Because of the rotational symmetry, the spectral function only depends on the magnitude $p \equiv |\mbf p|$ and the spatial vector components reduce to 
\begin{align}
 \rho^V_i(\mbf p) = \frac{p_i}{E_p}\,\rho_V
\end{align}
with $E_p = \sqrt{m^2 + p^2}$ and where $m$ is the effective mass consisting of the originally imposed mass and the Wilson parameter. Using $\rho_V \equiv -\rho_V^i E_p p_i / p^2$, we construct
\begin{align}
 \rho_+ \equiv \rho_V^0 + \rho_V\,, \quad \rho_- \equiv \rho_V^0 - \rho_V\,.
\end{align}
These functions correspond to positive and negative frequency operators
\begin{align}
 \Lambda_{\pm}(\mbf p) = \gamma^0 E_p + \gamma^j p_j \pm m\,,
\end{align}
with $j = 1,2,3$ and where $\Lambda_{\pm}(\mbf p) = \dfrac{1}{N_c} \sum_\lambda u_{\lambda,\mbf p}^{u/v}\, \bar{u}_{\lambda,\mbf p}^{u/v}$. In both the free case and in the HTL expression below, the spectral function can be decomposed in the frequency domain accordingly as
\begin{align}
 \label{eq_rho_Lambda_decomp_HTL}
 \rho^{\HTL}(\omega,\mbf p) = \dfrac{1}{2 E_p} \left( \Lambda_+(\mbf p)\,\rho_+(\omega,p) + \Lambda_-(-\mbf p)\,\rho_-(\omega,p) \right).
\end{align}
In this work, we consider almost massless fermions, such that we will disregard $\rho_S$ in the following and mostly focus on $\rho_{\pm}$.%
\footnote{Although we have to use a finite mass for technical reasons, it is taken to be small, such that the extracted spectral function can be compared to HTL calculations. However, a scalar component $\rho_S$ still arises due to the small mass value, which we will not discuss further in this work.}
